The Impact of Text Presentation on Translator Performance

Widely used computer-aided translation (CAT) tools divide documents into segments such as sentences and arrange them in a side-by-side, spreadsheet-like view. We present the first controlled evaluation of these design choices on translator performance, measuring speed and accuracy in three experimental text processing tasks. We find significant evidence that sentence-by-sentence presentation enables faster text reproduction and within-sentence error identification compared to unsegmented text, and that a top-and-bottom arrangement of source and target sentences enables faster text reproduction compared to a side-by-side arrangement. For revision, on the other hand, our results suggest that presenting unsegmented text results in the highest accuracy and time efficiency. Our findings have direct implications for best practices in designing CAT tools.

==> Target 2020 Final/commands.tex <==
% .tex file inclusion
\newcommand{\insertchapter}[1]{\input{chapters/#1}}

% references inside the document
\newcommand{\see}[1]{(see #1)}
\newcommand{\Chapter}[1]{Chapter~\ref{chap:#1}}
\newcommand{\Appendix}[1]{Appendix~\ref{chap:Appendix#1}}
\newcommand{\Section}[1]{Section~\ref{sec:#1}}
\newcommand{\Table}[1]{Table~\ref{tab:#1}}
\newcommand{\Figure}[1]{Figure~\ref{fig:#1}}
\newcommand{\Eq}[1]{Equation~\ref{eq:#1}}
\newcommand{\Eqp}[1]{(Equation~\ref{eq:#1})}
\newcommand{\Page}[1]{Page~\pageref{#1}}

% misc
\newcommand{\straightdoublequote}{\char"0022\relax}

% shortcuts
\newcommand{\ie}{i.e.\xspace}
\newcommand{\Ie}{I.e.\xspace}
\newcommand{\eg}{e.g.\xspace}
\newcommand{\Eg}{E.g.\xspace}
\newcommand{\ia}{inter alia}
\newcommand{\ibid}{\textit{ibid.}\xspace}
\newcommand{\Ibid}{\textit{Ibid.}\xspace}
\newcommand{\percent}{\,\%\xspace}
\newcommand{\etc}{\ldots\xspace}
\newcommand{\sic}{[sic]\xspace}
\newcommand{\vs}{\textit{vs.}\ }
\newcommand{\p}{$\circ$\xspace} % p < 0.1
\newcommand{\pp}{$\bullet$\xspace} % p < 0.05
\newcommand{\ppp}{$\bullet\,\bullet$\xspace} % p < 0.01
\newcommand{\pppp}{$\bullet\bullet\bullet$\xspace} % p < 0.001
\newcommand{\plus}{$+$}
\newcommand{\minus}{$-$}
\newcommand{\example}[1]{\textit{#1}}

% citation
\newcommand{\citeg}[1]{\citeauthor{#1}'s \citeyearpar{#1}} % cite genitive: Martinez et al's (2012)...

\newcommand{\Copy}{\textsc{Copy}\xspace}
\newcommand{\SC}{\Copy}
\newcommand{\Scan}{\textsc{Scan}\xspace}
\newcommand{\TC}{\Scan}
\newcommand{\Revise}{\textsc{Revise}\xspace}
\newcommand{\TR}{\Revise}



==> Target 2020 Final/tables/ResultsOverall.tex <==
\small
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{lllllllllllll}
\toprule
Task              && \multicolumn{2}{l}{\Copy} && \multicolumn{2}{l}{\Scan} && \multicolumn{2}{l}{\Revise: Named Entity} && \multicolumn{2}{l}{\Revise: Anaphor} \\[0.5em]
Response Variable && Speed      & Accuracy   && Speed    & Accuracy     && Speed           & Accuracy         && Speed          & Accuracy         \\
Unit              && words/h    & \# typos   && s/item   & \percent correct   && words/h         & \percent correct       && words/h        & \percent correct       \\ 
Sample Size       && 226        & 226        && 413      & 636          && 63              & 99              && 57             & 119              \\[0.5em] %\midrule
\multicolumn{9}{l}{\it Mean Response}                                                                                                              \\[0.2em]
Sentence, left--right (SL)               && 2,523.16   & 9.49       && 114.31   & 66.46        && 5,037.84        & 61.54            && 4,693.47       & 48.27            \\
Sentence, top--bottom (ST)               && 2,639.13   & 8.07       && 123.80   & 69.38        && 4,323.27        & 76.00            && 4,511.23       & 37.93            \\
Document, left--right (DL)               && 2,463.37   & 9.19       && 153.98   & 65.19        && 4,786.27        & 70.83            && 5,350.81       & 56.67            \\
Document, top--bottom (DT)               && 2,459.79   & 9.28       && 145.83   & 68.75        && 4,365.75        & 66.67            && 4,778.32       & 58.07            \\[0.5em] %\midrule
\multicolumn{9}{l}{\it Effects}                                                                                                                    \\[0.2em]
Segmentation      && \pppp &          && \ppp  &          &&       &       &&       & \p    \\
Orientation       && \pp   &          &&       &          && \ppp  &       &&       &       \\
Experience with MT && $n/a$ & $n/a$   && \ppp  & \pppp    && $n/a$ & \pp   && $n/a$ &       \\
Type of Manipulation && $n/a$ & $n/a$    && \pppp & \pppp    && $n/a$ & $n/a$ && $n/a$ & $n/a$ \\
\bottomrule
\end{tabular}

==> Target 2020 Final/tables/ReviseExamples.tex <==
\small
\raggedright

\begin{subtable}{\textwidth}
    \begin{tabularx}{\textwidth}{p{3mm}X}
        \toprule
        $S$    & \etc to an Earls Court apartment in 2014. It is on the first floor of a smart Queen Anne terrace - and it is a testament to the new design \etc \\
        $T_o$  & \etc zu einem Earls Court Apartment. Es liegt im ersten Stock einer eleganten Queen Anne Terrasse - und es ist ein Beweis für das neue Design \etc \\
        $T_m$  & \etc zu einem Earls Court Apartment. Sie liegt im ersten Stock einer eleganten Queen Anne Terrasse - und es ist ein Beweis für das neue Design \etc \\
        \bottomrule
    \end{tabularx}
    \caption{Anaphor}
    \label{tab:Exp2ReviseExamplesAnaphora}
    \vspace{1em}
\end{subtable}

\begin{subtable}{\textwidth}
    \begin{tabularx}{\textwidth}{p{2mm}X}
        \toprule
        $S$    & Pokémon Go, a worthy hunt for health and happiness \etc Within days, Pokémon Go had more users than Tinder \etc But the beauty of Pokémon Go is it gets people outside doing something they enjoy \etc \\
        $T_o$  & Pokémon Go, eine Jagd nach Gesundheit und Glück, die sich lohnt \etc Innerhalb weniger Tage hatte Pokémon Go mehr Benutzer als Tinder \etc Aber das Wundervolle an Pokémon Go ist, dass es die Leute dazu bringt, etwas im Freien zu tun \etc  \\
        $T_m$  & Pokémon Go, eine Jagd nach Gesundheit und Glück, die sich lohnt \etc Innerhalb weniger Tage hatte Pokémon Go mehr Benutzer als Tinder \etc Aber das Wundervolle an Pokémon Gehen ist, dass es die Leute dazu bringt, etwas im Freien zu tun \etc  \\
        \bottomrule
    \end{tabularx}
    \caption{Named Entity}
    \label{tab:Exp2ReviseExamplesNamedEntity}
    \vspace{1em}
\end{subtable}

==> Target 2020 Final/tables/ScanExamples.tex <==
\small
\raggedright

\begin{subtable}{\textwidth}
    \begin{tabularx}{\textwidth}{p{2mm}X}
        \toprule
        $S$    & While sufferers are usually advised to dodge meat and dairy to soothe their symptoms, researchers at Washington University found protein's essential amino acid tryptophan helps develop immune cells that foster a tolerant gut.\\
        $T_o$  & Während den Betroffenen normalerweise geraten wird, Fleisch und Milchprodukte zu meiden, um ihre Symptome zu lindern, fanden Forscher an der Washingtoner Universität heraus, dass die essentielle Aminosäure Tryptophan von Proteinen dazu beiträgt, Immunzellen zu entwickeln, die einen toleranten Darm fördern. \\
        $T_m$  & Während den Betroffenen normalerweise geraten wird, Fleisch und Milchprodukte zu meiden, um ihre Symptome zu lindern zu lindern zu lindern, fanden Forscher an der Washingtoner Universität heraus, dass die essentielle Aminosäure Tryptophan von Proteinen dazu beiträgt, Immunzellen zu entwickeln, die einen toleranten Darm fördern. \\
        \bottomrule
    \end{tabularx}
    \caption{Addition}
    \label{tab:Exp2ScanExamplesAddition}
    \vspace{1em}
\end{subtable}

\begin{subtable}{\textwidth}
    \begin{tabularx}{\textwidth}{p{3mm}X}
        \toprule
        $S$    & Patrick Roy resigned as coach and vice president of the hockey operations of the Colorado Avalanche on Thursday, citing a lack of a voice within the team's decision-making process. \\
        $T_o$  & Patrick Roy trat am Donnerstag als Trainer und Vice President Of Hockey Operations der Colorado Avalanche zurück und führte ein zu geringes Mitbestimmungsrecht beim Entscheidungsprozess des Teams an. \\
        $T_m$  & Patrick Roy trat am Donnerstag als Trainer und Vice President Of Hockey Operations zurück und führte ein zu geringes Mitbestimmungsrecht beim Entscheidungsprozess des Teams an. \\
        \bottomrule
    \end{tabularx}
    \caption{Omission}
    \label{tab:Exp2ScanExamplesOmission}
    \vspace{1em}
\end{subtable}

\begin{subtable}{\textwidth}
    \begin{tabularx}{\textwidth}{p{3mm}X}
        \toprule
        $S$    & Heavy rain, flooding prompts rescues in Louisiana, Mississippi \\
        $T_o$  & Heftige Regenfälle, Überschwemmung gibt Anlass zu Rettungen in Louisiana, Mississippi \\
        $T_m$  & Öffnen Sie im zweiten Fenster das eigene Persönliche Verzeichnis. \\
        \bottomrule
    \end{tabularx}
    \caption{Wrong Meaning}
    \label{tab:Exp2ScanExamplesWrongMeaning}
    \vspace{1em}
\end{subtable}

\begin{subtable}{\textwidth}
    \begin{tabularx}{\textwidth}{p{3mm}X}
        \toprule
        $S$    & The ``Made in America'' event was designated an official event by the White House, and would not have been covered by the Hatch Act. \\
        $T_o$  & Die Veranstaltung ``Made in America'' wurde vom Weißen Haus als offizielle Veranstaltung bezeichnet und wäre nicht vom Hatch Act abgedeckt worden. \\
        $T_m$  & Die Veranstaltung ``Made in America'' wurde vom Weißen Haus als offizielle Veranstaltung bezeichnet und wäre nicht vom Hatch Act abgedeckt worden. \\
        \bottomrule
    \end{tabularx}
    \caption{No Error}
    \label{tab:Exp2ScanExamplesNoError}
    \vspace{1em}
\end{subtable}


==> Target 2020 Final/tables/Surveys.tex <==
\centering

% \begin{subtable}{\textwidth}
%     \centering
%     \begin{tabular}{lr}
%     \toprule
%         min    & 1.00  \\
%         max    & 28.00 \\
%         mean   & 10.70 \\
%         median & 6.50  \\
%     \bottomrule
%     \end{tabular}
%     \caption{Full-time professional experience}
%     \label{tab:Exp2SurveysExperience}
% \end{subtable}

% \bigskip

\begin{subtable}{\textwidth}
    \centering
    \begin{tabular}{lrrrrr}
    \toprule
                               & None & Courses & Bachelor's & Master's & PhD \\ \midrule
        Translation            & 5    & 3       & 7          & 4        & 1   \\
        Information Technology & 10   & 9       & 0          & 1        & 0   \\
    \bottomrule
    \end{tabular}
    \caption{Education (highest degree)}
    \label{tab:Exp2SurveysEducation}
\end{subtable}

\bigskip

\begin{subtable}{\textwidth}
    \centering
    \begin{tabular}{lrrr}
    \toprule
                               & Regular & Sometimes & Never \\ \midrule
        Translation Memory     & 15      & 4         & 1     \\
        Terminology Management & 7       & 9         & 4     \\
        Machine Translation    & 5       & 10        & 5     \\
        Quality Assurance      & 4       & 8         & 8     \\
    \bottomrule
    \end{tabular}
    \caption{Use of translation technology}
    \label{tab:Exp2SurveysUse}
\end{subtable}

% \bigskip

% \begin{subtable}{\textwidth}
%     \centering
%     \begin{tabular}{lrrrrr}
%     \toprule
%                                     & SL & ST & Sx & DL & DT \\ \midrule
%         Commercial (pre-experiment) & 17 & 1  & 2  &    &    \\
%         \Copy (post-task)           & 3  & 13 &    & 3  & 1  \\
%         \Scan (post-task)           & 7  & 10 &    & 3  & 0  \\
%         \Revise (post-task)         & 6  & 10 &    & 3  & 1  \\
%         Overall (post-experiment)   & 3  & 13 &    & 3  & 1  \\
%     \bottomrule
%     \end{tabular}
%     \caption{Preferred text presentation: sentence (S) or document (D) segmentation with left--right (L), top--bottom (T), or any (x) orientation.}
%     \label{tab:Exp2SurveysPrefs}
% \end{subtable}
